Kaskade: Graph Views for Efficient Graph Analytics

Graphs are an increasingly popular way to model real-world entities and relationships between them, ranging from social networks to data lineage graphs and biological datasets. Queries over these large graphs often involve expensive subgraph traversals and complex analytical computations. These real-world graphs are often substantially more structured than a generic vertex-and-edge model would suggest, but this insight has remained mostly unexplored by existing graph engines for graph query optimization purposes. Therefore, in this work, we focus on leveraging structural properties of graphs and queries to automatically derive materialized graph views that can dramatically speed up query evaluation. We present KASKADE, the first graph query optimization framework to exploit materialized graph views for query optimization purposes. KASKADE employs a novel constraint-based view enumeration technique that mines constraints from query workloads and graph schemas, and injects them during view enumeration to significantly reduce the search space of views to be considered. Moreover, it introduces a graph view size estimator to pick the most beneficial views to materialize given a query set and to select the best query evaluation plan given a set of materialized views. We evaluate its performance over real-world graphs, including the provenance graph that we maintain at Microsoft to enable auditing, service analytics, and advanced system optimizations. Our results show that KASKADE substantially reduces the effective graph size and yields significant performance speedups (up to 50X), in some cases making otherwise intractable queries possible.

==> Makefile <==
LATEX=pdflatex  # or latex, xelatex, whichever you have
LATEXOPT=--shell-escape  # needed for \usepackage{minted}
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf
CONTINUOUS=-pvc

# TODO: Add tikz figures here.
MAIN=paper
SOURCES=$(MAIN).tex Makefile sections/*tex
FIGURES := $(shell find figures/* images/* -type f)

# Default just builds it once (continuous mode disabled for latexmk).
all:	once

# Use make debug to view errors when latexmk is running in continuous mode.
continuous:	$(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) -pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

force:
	touch .refresh
	rm $(MAIN).pdf
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
	$(LATEXMK) -C
	rm -f $(MAIN).pdfsync
#	rm -rf *~ *.tmp
	rm -rf _minted-paper/
	rm -f *.aux *.dvi *.log *.blg *.bbl *-blx.bib *.xml

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

debug:
	$(LATEX) $(LATEXOPT) $(MAIN)

.PHONY: clean force once all


==> figures/Makefile <==
all: spanner_view-a.pdf spanner_view-b.pdf

spanner_view-%.pdf:
	for f in *tex ; do \
		pdflatex -shell-escape $$f ; \
	done

clean:
	rm -f spanner_view-?.{pdf,aux,log}

